An Almost Singularly Optimal Asynchronous Distributed MST Algorithm

A singularly (near) optimal distributed algorithm is one that is (near) optimal in \emph{two} criteria, namely, its time and message complexities. For \emph{synchronous} CONGEST networks, such algorithms are known for fundamental distributed computing problems such as leader election [Kutten et al., JACM 2015] and Minimum Spanning Tree (MST) construction [Pandurangan et al., STOC 2017, Elkin, PODC 2017]. However, it is open whether a singularly (near) optimal bound can be obtained for the MST construction problem in general \emph{asynchronous} CONGEST networks. We present a randomized distributed MST algorithm that, with high probability, computes an MST in \emph{asynchronous} CONGEST networks and takes $\tilde{O}(D^{1+\epsilon} + \sqrt{n})$ time and $\tilde{O}(m)$ messages, where $n$ is the number of nodes, $m$ the number of edges, $D$ is the diameter of the network, and $\epsilon >0$ is an arbitrarily small constant (both time and message bounds hold with high probability). Our algorithm is message optimal (up to a polylog$(n)$ factor) and almost time optimal (except for a $D^{\epsilon}$ factor). Our result answers an open question raised in Mashregi and King [DISC 2019] by giving the first known asynchronous MST algorithm that has sublinear time (for all $D = O(n^{1-\epsilon})$) and uses $\tilde{O}(m)$ messages. Using a result of Mashregi and King [DISC 2019], this also yields the first asynchronous MST algorithm that is sublinear in both time and messages in the $KT_1$ CONGEST model. A key tool in our algorithm is the construction of a low diameter rooted spanning tree in asynchronous CONGEST that has depth $\tilde{O}(D^{1+\epsilon})$ (for an arbitrarily small constant $\epsilon > 0$) in $\tilde{O}(D^{1+\epsilon})$ time and $\tilde{O}(m)$ messages. To the best of our knowledge, this is the first such construction that is almost singularly optimal in the asynchronous setting.

==> app-spanning-tree.tex <==

We first provide definitions and an auxiliary lemma (see Lemma \ref{lem:MPXArrivals}) followed by proofs of Lemmas \ref{lem:mpxDecomp} and \ref{lem:MPXDiameter}, stated in Section \ref{ss:MPX}. After which, we provide the proofs of Lemma \ref{lem:diameterOfClustersAndClusterGraph} and Corollary \ref{cor:finalClusterGraph}, stated in Section \ref{sec:rootedSpanningTree}.

Consider some fixed execution of the algorithm and node $v \in \overline{V}$. Then $D_u = S_u + dist(u,v) - 1 = \delta_{max} - \lfloor \delta_u \rfloor + dist(u,v) - 1$ denotes the \emph{(arrival) round} of $u$, that is, the first round in which $v$ can receive a message from $u$'s cluster. 
For every integer $1 \leq j \leq n$, let $z_j$ be the node with the $j$th smallest arrival round in the execution. For every integer $1 \leq k \leq n$, let  $S_k=\{z_1,\ldots,z_k\}$. Building upon these definitions, for a node $v \in \overline{V}$, positive integers $1 \leq k,r \leq n$, let $\EV_{v,k,r}$ denote the event that after the execution of the algorithm, $D_{z_{k+1}} - D_{z_1} \leq r$.

\begin{lemma}
\label{lem:MPXArrivals}
For any node $v \in \overline{V}$ and positive integers $1 \leq k,r \leq n$, 
$$\Pr(\EV_{v,k,r}) ~\le~ (1 - \exp(- (r+1) \beta))^k$$
\end{lemma}

\begin{proof}
We condition on $S_k$ and $D^*=D_{z_{k+1}}$. The proof is based on first showing the stated upper bound on the probability of $\EV_{v,k,r}$ conditioned on $S_k$ and $D^*$, and then applying the law of total probability to derive the lemma statement. We next describe the first half of the proof in more detail.

For any integer $i \geq 1$, let $c_{z_i} = \delta_{max} + dist(z_i,v) - 1$. We have
$\Pr(\EV_{v,k,r} \; | \; S_k, D^*)\le p$ for
$$p ~=~ \Pr\left(\bigwedge_{i=1}^k [D^* - D_{z_i} \leq r]\right) ~=~ \Pr\left(\bigwedge_{i=1}^k [\delta_{z_i} \leq r + 1 +c_{z_i} - D^*]\right) ~=~ \prod_{i=1}^k \Pr(\delta_{z_i} \leq r + 1 +c_{z_i} - D^*),$$ 
where the last equality holds since the random variables $\delta_{z_i}$ are independent. 
Next, note that $D^* \geq D_{z_i}$ for any integer  $1 \leq i \leq k$, and thus $\Pr(\lfloor \delta_{z_i} \rfloor \geq c_{z_i} - D^*) = 1$. Hence, $\Pr(\delta_{z_i} \geq c_{z_i} - D^*) = 1$ and 
$$p ~=~ \prod_{i=1}^k \Pr(\delta_{z_i} \leq r +1 + c_{z_i} - D^* \; | \; \delta_{z_i} \geq c_{z_i} - D^*).$$ 
Finally,  
$$p ~\leq~ \prod_{i=1}^k \Pr(\delta_{z_i} \leq r+1) ~=~ \prod_{i=1}^k (1 - \exp(- (r+1) \beta)) ~=~ (1 - \exp(- (r+1) \beta))^k$$
where the inequality holds by the memorylessness of the exponential distribution.
\end{proof}


\begin{proof}[Proof of Lemma \ref{lem:mpxDecomp}]
We first note for any node $v \in \overline{V}$, $\Pr[\lfloor \delta_v \rfloor > \delta_{max}] = \Pr[\delta_v > \frac{2 \ln n}{\beta}] = \exp(- 2 \ln n) = \frac{1}{n^2}$. Hence, by union bound, $\lfloor \delta_v \rfloor \leq \delta_{max}$ for every node $v \in \overline{V}$ with high probability. We hereafter exclude this unlikely event and assume $\delta_{max} \geq \max_{v \in \overline{V}} \{\lfloor \delta_v \rfloor\}$. This implies that all nodes belong to a cluster.

Next, note that by the algorithm description, each cluster is spanned by a tree of depth at most $\frac{2 \ln n}{\beta}$. Hence, all clusters have strong diameter at most $\frac{4 \ln n}{\beta}$.
Finally, an edge is cut if its two endpoints $u$ and $v$ are in different clusters. This implies that for node $v$ (without loss of generality), the two smallest arrival rounds differ by at most 1, which corresponds to event $\EV_{v,1,1}$. By Lemma \ref{lem:MPXArrivals}, $\Pr(\EV_{v,1,1}) \leq (1 - \exp(- 2\beta)) \leq 2 \beta$. The lemma follows.
\end{proof}

\begin{proof}[Proof of Lemma \ref{lem:MPXDiameter}]
Again, we assume $\delta_{max} \geq \max_{u \in \overline{V}} \{\delta_u\}$, which holds with high probability. For any node $v \in \overline{V}$, let $C_v$ denote the cluster containing $v$ after the execution of the algorithm.

Consider any two nodes $u,v \in \overline{V}$ such that $l = dist_{\overline{G}}(u,v) > 3 \beta \overline{D}$. (Note that if $l \leq 3 \beta \overline{D}$, then $dist_{\overline{G}^*}(C_u,C_v) \leq 3 \beta \overline{D}$.)
Let $(w_1,\ldots,w_{l+1})$ be the shortest path  between $u$ and $v$ in $\overline{G}$ (where $w_1 = u$ and $w_{l+1} = v$). Moreover, for any integer $i \in [1,l]$, let $X_i$ be the indicator random variable of $w_i$ and $w_{i+1}$ being in the same cluster. Then, the random variable $X = \sum_{i=1}^{l} X_i$ is an upper bound on $dist_{\overline{G}^*}(C_u,C_v)$. By Lemma \ref{lem:mpxDecomp}, each edge is an inter-cluster edge with probability at most $2\beta$. Hence, by the linearity of expectation, $E[X] \leq 2\beta l$.

Next, let us provide a concentration bound for $X$ by showing that the random variables $X_i$ are only locally dependent. First, for any two integers $i, j \in [1,l]$ such that $|i - j| > \lfloor 4 \frac{\ln n}{\beta} \rfloor$, $X_i$ and $X_j$ are independent (since the same node cannot affect $w_i$ and $w_j$ with our choice of $\delta_{max}$). Then, we can color the random variables $\{X_i\}_{i=1,\ldots,l}$ using $\chi = \lfloor 4 \frac{\ln n}{\beta} \rfloor$ --- by coloring $X_i$ with $i \mod (\chi + 1)$ --- such that variables with the same color are independent. In other words, the random variables $X_i$ are only locally dependent and thus we can apply a specific Chernoff-Hoeffding bound (Theorem 3.2 from \cite{DP09}): $\Pr(X \geq E[X] + t)  \leq \exp(-2t^2 / (\chi \cdot l))$. Hence, $\Pr(X \geq 3 \beta l)  \leq \exp(-2 (\beta l)^2 / (\chi \cdot l)) \leq \exp(-2 \beta^2 l /\chi)$.
Since $l > 3 \beta \overline{D} > 3 k \frac{\ln^2 n}{\beta^3}$, $\Pr(X \geq 3 \beta l) \leq \exp(- \frac{3}{2} k \ln n) \leq \frac{1}{n^k}$. By taking a union bound over all $n^2$ possible pairs of nodes $u,v \in \overline{V}$, the lemma statement follows.
\end{proof}



\begin{proof}[Proof of Lemma \ref{lem:diameterOfClustersAndClusterGraph}]
By induction on $i$. The base case, $i = 1$, holds trivially. 

Next, consider some $i \geq 1$ for which the inductive hypothesis holds, i.e., $\diam(G_{i-1})=\max\{ (3 \beta)^{i-1} D, O(\log^{2+4/\epsilon'} n)\}$ w.h.p. and each cluster node $C$ of the partition $\mathcal{P}_{i-1}$ is spanned (in the original graph $G$) by a tree $\CLT(C)$ with $\diam(\CLT(C))= (\frac{5 \ln n}{\beta})^{i-1}$. Running Procedure~$\MPX$ on $G_{i-1}$ yields a $(2\beta, \frac{4 \ln n}{\beta})$ low-diameter decomposition of $G_{i-1}$. In fact, each super cluster $C'$ of this decomposition on $G_{i-1}$ is spanned (in the cluster graph $G_{i-1}$) by a tree $\CLT(C')$ of diameter $\frac{4 \ln n}{\beta}$. 
Hence, the ``combined'' spanning tree computed by Procedure~$\Transform$ for the ``analog'' $C''$ of cluster $C'$ on $G$, which is a cluster of the newly constructed $G_i$, has diameter $\diam(\CLT(C''))= (\frac{4 \ln n}{\beta} + 1) \cdot (\frac{5 \ln n}{\beta})^{i-1} \leq  (\frac{5 \ln n}{\beta})^{i}$. Next, the diameter of $G_i$ is the same as that of the cluster graph $H$ induced by partition $\mathcal{P}_i^*$. By Lemma \ref{lem:MPXDiameter}, the diameter of $H$ is $\max\{ (3 \beta)^{i} D, O(\log^{2+4/\epsilon'} n)\}$ w.h.p., and thus the lemma statement holds.
\end{proof}

\begin{proof}[Proof of Corollary \ref{cor:finalClusterGraph}]
By Lemma \ref{lem:diameterOfClustersAndClusterGraph} (and applying one extra induction step), the diameter of $G_{\imax}$ is $D_f = \max\{ (3 \beta)^{\imax} D, O(\log^{2+4/\epsilon'} n)\}$ and each cluster $C$ of the partition $\mathcal{P}_{\imax}$ is spanned in $G$ by a tree $\CLT(C)$ of depth $d_f = (\frac{5 \ln n}{\beta})^{\imax}$. Since $\imax = \lceil \log_{1/(3\beta)} D \rceil$, we have that $(3 \beta)^{\imax} \leq 1/D$, so $D_f = O(\log^{2+4/\epsilon'} n)$. Moreover, by going through the computations, we get: 
\begin{align*}
d_f &=~  \exp(\imax \ln(5 \ln^{1+1/\epsilon'} n)) 
~\leq~  (5 \ln^{1+1/\epsilon'} n)  \exp\left(\frac{\ln D \ln(5 \ln^{1+1/\epsilon'} n)}{\ln(\frac{1}{3} \ln^{1/\epsilon'} n) }\right)  
&\\
&=~ (5 \ln^{1+1/\epsilon'} n)   \exp\left(\ln D \cdot \frac{\ln 5 + (1+1/\epsilon') \ln\ln n}{\frac{1}{\epsilon'} \ln\ln n - \ln 3}\right) &\\
&=~  (5 \ln^{1+1/\epsilon'} n)  \exp\left(\ln D \cdot \left(1 + \frac{\ln 5 + \ln 3 + \ln\ln n}{ \frac{1}{\epsilon'} \ln\ln n - \ln 3}\right)\right)
&\\
&\leq~  (5 \ln^{1+1/\epsilon'} n) \exp(\ln D \cdot (1 + 2\epsilon' \ln 15 )) 
~\leq~  (5 \ln^{1+1/\epsilon'} n) ~ D^{1 + \epsilon}~, 
\end{align*}
where, in order to make the last inequality hold, Procedure~$\SpanningTreeConstruction(\epsilon)$ selects $\epsilon' \leq \epsilon / (2\ln 15)$.
\end{proof}
